Visual-Inertial Target Tracking and Motion Planning for UAV-based Radiation Detection

This paper addresses the problem of detecting radioactive material in transit using an UAV of minimal sensing capability, where the objective is to classify the target's radioactivity as the vehicle plans its paths through the workspace while tracking the target for a short time interval. To this end, we propose a motion planning framework that integrates tightly-coupled visual-inertial localization and target tracking. In this framework,the 3D workspace is known, and this information together with the UAV dynamics, is used to construct a navigation function that generates dynamically feasible, safe paths which avoid obstacles and provably converge to the moving target. The efficacy of the proposed approach is validated through realistic simulations in Gazebo.

==> Observability.tex <==
\section{Appendix}

\subsection{Appendix A: Target Tracking Noise Covariance}

%
The state transition matrix for the target state is given by ($\Delta t = t_{k+1}-t_k$):
\begin{align}
\mathbf{A}(t_{k+1},t_k) = \begin{bmatrix} \mathbf{I} & \Delta t\mathbf{I} & \frac{1}{2}\Delta t^2 \mathbf{I} & \cdots & \frac{1}{N!}\Delta t^{N}\mathbf{I} \\ \mathbf{0} & \mathbf{I} & \Delta t \mathbf{I} & \cdots & \frac{1}{(N-1)!}\Delta t^{N-1}\mathbf{I} \\
\mathbf{0} & \mathbf{0} & \mathbf{I} & \cdots & \frac{1}{(N-2)!}\Delta t^{N-2}\mathbf{I} \\ \vdots & \vdots & \vdots & \ddots & \vdots \\
\mathbf{0} & \mathbf{0} & \mathbf{0} & \cdots & \mathbf{I}  
\end{bmatrix}
\end{align}
%
The discrete noise covariance is given by:
\begin{align}
\mathbf{Q}_{Td} & = \int_{t_k}^{t_{k+1}} \mathbf{A}(t_{k+1}, \tau) \mathbf{G}\mathbf{Q}_{Tc} \mathbf{G}^{\top} \mathbf{A}(t_{k+1}, \tau)^{\top} d\tau \\
\mathbf{Q}_{Tc} &= \sigma_{Tc}^2\mathbf{I}
\end{align}
Defining $\delta t= t_{k+1} -\tau$:
\begin{align}
\mathbf{Q}_{Td} &= \sigma_{Tc}^2\int_{0}^{\Delta t}  \mathbf{B}(\delta t) \mathbf{B}(\delta t)^{\top} d\delta t\\
\mathbf{B}(\delta t) &= \begin{bmatrix} \frac{1}{N!}\delta t^{N}\mathbf{I}\ \\ \frac{1}{(N-1)!}\delta t^{N-1}\mathbf{I} \\ \frac{1}{(N-2)!}\delta t^{N-2}\mathbf{I} \\ \vdots \\ \mathbf{I} \end{bmatrix} \\
\end{align}
From which we can see that the $i,jth$ block entry of the covariance matrix (with zero-indexing) will be given by:
\begin{align}
\mathbf{Q}_{ij} = \frac{\sigma_{TC}^2\Delta t^{2N-i-j+1}}{(N-i)!(N-j)!(2N-i-j+1)}\mathbf{I} 
\end{align}




\subsection{Appendix B: Observability}
Here we present the observability results for a monocular VINS system tracking a moving target. For a background in the observability study of VINS, we refer the reader to~\cite{Hesch2013TRO}.  
The kth row of the observability matrix for an IMU-camera aligned robot and a moving target system (parameterized up to order n) is given by:
\begin{align}
\mathbf{M}_k &= \mathbf{H}_k{\bm \Psi}(k, 1) \nonumber\\
& \begin{matrix}= \Gamma_1  (\Gamma_2 & \Gamma_3 & -\delta t\mathbf{I} & \Gamma_4 & -\mathbf{I} & \mathbf{I} & \delta t\mathbf{I} &  \frac{1}{2}\delta t^2  \mathbf{I} \\ \cdots & \frac{1}{n!}\delta t^n \mathbf{I})  \end{matrix} \\
%
\Gamma_1 &= \mathbf{H}_{c,k}{}_G^{I_k}\mathbf{R} \\
\Gamma_2 &= \lfloor {}^G\mathbf{p}_{T_k}-  {}^G\mathbf{p}_{I_1} - {}^G\mathbf{v}_{I_1}\delta t+ \frac{1}{2}{}^G\mathbf{g} \delta t^2 \rfloor{}_{I_1}^G \mathbf{R} \nonumber\\
&= \lfloor {}^G\mathbf{p}_{T_1}+ \sum_{i=1}^{n} \frac{1}{i!}(\delta t^i) {}^G\mathbf{p}^{(i)}_{T_1}-  {}^G\mathbf{p}_{I_1} - \nonumber\\ &{}^G\mathbf{v}_{I_1}\delta t+ \frac{1}{2}{}^G\mathbf{g} \delta t^2 \rfloor{}_{I_1}^G \mathbf{R} \\
%
\Gamma_3 &=  \lfloor {}^G\mathbf{p}_{T_k}-  {}^G\mathbf{p}_{I_k} \rfloor{}_{I_k}^G \mathbf{R}\int_{t_1}^{t_k}\left(-{}_{I_s}^{I_k} \mathbf{R}\right)ds -  \\ &\int_{t_1}^{t_k}\int_{t_1}^{\theta}{}_{I_s}^{G}\mathbf{R}\lfloor {}^{I_s}\mathbf{a} \rfloor\int_{t_1}^s{}_{I_{\tau}}^{I_s}\mathbf{R}d\tau ds d\theta\\
%
\Gamma_4 &= \int_{t_1}^{t_k}\int_{t_1}^{s}{}_{I_\tau}^G\mathbf{R}d\tau ds 
\end{align}
%
where ${\bm \Psi}(k, 1)$ is the state-transition matrix of the robot-target system between steps 1 and k and $\mathbf{H}_k$ is the Jacobian matrix for the kth robot to target bearing measurement occuring at time $\delta t$.

This yields the following unobservable directions:
\begin{align}
\mathbf{N_1} &= \begin{bmatrix} \mathbf{0}_3 \\ \mathbf{0}_3 \\\mathbf{0}_3 \\\mathbf{0}_3 \\ \mathbf{I}_3 \\\mathbf{I}_3  \\ \mathbf{0}_3 \\ \vdots \\ \mathbf{0}_3 \end{bmatrix} &
%
\mathbf{N_2} &= \begin{bmatrix} {}_G^{I_1}\mathbf{R}{}^G\mathbf{g} \\ \mathbf{0}_3 \\-\lfloor{}^G\mathbf{v}_{I_1}\rfloor^G\mathbf{g} \\ \mathbf{0}_3 \\-\lfloor{}^G\mathbf{p}_{I_1}\rfloor^G\mathbf{g}  \\-\lfloor{}^G\mathbf{p}_{T_1}\rfloor^G\mathbf{g} \\ -\lfloor {}^G\mathbf{p}^{(1)}_{T_1}\rfloor^G\mathbf{g} \\ \vdots \\ -\lfloor {}^G\mathbf{p}^{(N)}_{T_1}\rfloor^G\mathbf{g}  \end{bmatrix} &
%
\mathbf{N_3} &= \begin{bmatrix} \mathbf{0}_3 \\ \mathbf{0}_3 \\\mathbf{I}_3 \\\mathbf{0}_3 \\ \mathbf{0}_3 \\\mathbf{0}_3  \\ \mathbf{I}_3 \\ \mathbf{0}_3 \\ \vdots \\ \mathbf{0}_3 \end{bmatrix} 
\end{align}
%
So we can see that, in addition to the classic unobservable directions of VINS with static features, the initial global velocity of the total system is unobservable. Note that when using both targets and features, the total number of unobservable directions is reduced to four ($\mathbf{N}_1,\mathbf{N}_2$)  , as this is the intersection of the nullspace of the two measurement types.
%

\subsection{Appendix C: Required Number of Bearing Measurements to Recover Target State}

In the case where VINS has access to static feature measurements, the position and orientation of the system can be recovered in a fixed-global position and yaw frame. If, at M different measuring times, the robot receives bearing measurements which can be rotated back into the global frame, then the constraint satisfied at time i is given by:
%
\iffalse
\begin{align}
\mathbf{p}_R (i) &= -d_i \mathbf{b}_i +\mathbf{p}_T(0)+ \Delta t_i \dot{\mathbf{p}}_{T_0}+ \frac{1}{2}\Delta t_i^2 \ddot{\mathbf{p}}_T(0) + \cdots + \nonumber \\ 
&\frac{1}{(N-1)!}\Delta t_i^{N-1} \frac{\partial^{N-1}}{\partial t^{N-1}} {\mathbf{p}}_T(0)
\end{align}
\fi
\begin{align}
{}^G\mathbf{p}_{c_i} &= -d_i \mathbf{b}_i +{}^G\mathbf{p}_{T_0}+ \Delta t_i {}^G\mathbf{p}^{(1)}_{T_0} \frac{1}{2}\Delta t_i^2 {}^G\mathbf{p}^{(2)}_{T_0} + \\ &\cdots +  
\frac{1}{(N)!}\Delta t_i^{N}  {}^G{\mathbf{p}}^{(N)}_{T_0}
\end{align}
%
Where ${}^G\mathbf{p}_{c_i},  d_i, \mathbf{b}_i, \Delta t_i$ are the position of the robot's camera in the global frame, depth of the target in the ith image, bearing from the robot to the target expressed in the global frame, and time since the first measurement at time i. ${}^G\mathbf{p}_{T_0}$ and its derivatives represent the initial position derivatives of the target. Note that we are using a constant position derivative model of arbitrary order. Stacking these equations and separating out the unknowns leads to:
%
\iffalse
\begin{align}
\begin{bmatrix} \mathbf{p}_R (0) \\ \mathbf{p}_R (1) \\ \mathbf{p}_R (2) \\ \vdots \\ \mathbf{p}_R (M) \end{bmatrix} &=  \mathbf{A} \begin{bmatrix} \mathbf{p}_T (0) \\ \dot{\mathbf{p}}_T (0) \\\ddot{\mathbf{p}}_T (0) \\ \vdots \\ d_0 \\ d_1 \\ \vdots \\ d_M \end{bmatrix} \\
\end{align}
\fi
%
\begin{align}
\begin{bmatrix} {}^G\mathbf{p}_{c_0} \\ {}^G\mathbf{p}_{c_1} \\ {}^G\mathbf{p}_{c_2} \\ \vdots \\ {}^G\mathbf{p}_{c_M} \end{bmatrix} &=  \mathbf{Y} \begin{bmatrix} {}^G\mathbf{p}_{T_0} \\ {}^G\mathbf{p}^{(1)}_{T_0} \\ {}^G\mathbf{p}^{(2)}_{T_0} \\ \vdots \\ d_0 \\ d_1 \\ \vdots \\ d_M \end{bmatrix} \\
\end{align}
%
Where the matrix $\mathbf{Y}$ is given by:
\begin{align}
 \begin{bmatrix}  \mathbf{I} & \mathbf{0} & \mathbf{0} & \cdots &  -\mathbf{b}_0 & \mathbf{0} & \mathbf{0} & \cdots & \mathbf{0}  \\\mathbf{I} & \Delta t_1 \mathbf{I} & \frac{1}{2}\Delta t_1^2 \mathbf{I} & \cdots &  \mathbf{0} & -\mathbf{b}_1 &\mathbf{0} &  \cdots & \mathbf{0} \\
\mathbf{I} & \Delta t_2 \mathbf{I} & \frac{1}{2}\Delta t_2^2 \mathbf{I} & \cdots &  \mathbf{0}  &\mathbf{0}& -\mathbf{b}_2 &  \cdots & \mathbf{0} \\
\vdots & \vdots &  \vdots & \ddots & \vdots & \vdots & \vdots & \ddots & \vdots \\
\mathbf{I} & \Delta t_M \mathbf{I} & \frac{1}{2}\Delta t_M^2 \mathbf{I} & \cdots &  \mathbf{0}  &\mathbf{0} &  \cdots & \cdots & -\mathbf{b}_M 
\end{bmatrix}
\end{align}
%
Which we can see is a linear system whose A matrix is of size $3M \times (3(N+1)+M)$ and is, in general, full rank. In order to fully constrain the system then, we need the measurements and derivative order such that $2M \geq 3(N+1)$. In particular, a constant position target requires 2 measurements, constant velocity requires 3, constant acceleration requires 5, etc. 

==> z_localization.tex <==
\subsection{Localization with a Prior Map}
In this work we wish to perform control using navigation functions within a known map. Therefore, the robot must be able to localize using bearing measurements to known landmarks. Hereafter we use the terms ``features" and ``landmarks" to distinguish between objects in the IMU's ``global" frame and objects with known positions in the "map" frame. In order to utilize these landmarks, we must estimate the transformation between the these two frames. We assume that the map and global frame align along their z-direction due to the observability of orientation in VINS up to rotations about the gravity vector. As such, the transformation only has 4 degrees of freedom: a relative position between the respective origins and a relative yaw. Formaly, we write it as the following relative orientation state and error state:
%
\begin{align}
{}_G^M \bar{q}&= 
\begin{bmatrix} 
 0 \\ 0 \\ \frac{\theta}{|\theta|}\sin{\frac{|\bm \theta|}{2}} \\ \cos{\frac{|\bm \theta|}{2}}
\end{bmatrix} = \begin{bmatrix} 
 0 \\ 0 \\ \frac{\psi}{2} \\ 1
\end{bmatrix} \otimes {}_G^M \hat{\bar{q}}
\end{align}

So we parameterize the relative orientation using a single DOF quaternion. All updates to this quaternion are achieved by further rotations about the z-axis. In addition to this orientation error we also estimate the relative position vector ${}^G \mathbf{p}_M$ which gives us the map origin in the global frame of reference. 

The function which maps the landmarks expressed in the map frame, ${}^M \mathbf{L}_f$,into the current camera takes the form:
%
\begin{align}
    \mathbf{z} &= \Pi({}^{C_k}\mathbf{L}_f) + \mathbf{n} \\
    {}^{C_k}\mathbf{p}_f &= {}^C_I\mathbf{R}{}^{I_k}_G\mathbf{R}\left( {}^G \mathbf{p}_M + {}^M_G \mathbf{R}^{\top} {}^M \mathbf{L}_f- {}^G\mathbf{p}_{I_k} \right) + {}^C \mathbf{p}_{I}
\end{align}
%
%
The measurement Jacobians are given by:
%
%
%
%
\begin{align}
    \mathbf{H}_{proj}&= \begin{bmatrix} \frac{1}{z} & 0 & -\frac{x}{z^2} \\ 0 & \frac{1}{z}  & -\frac{y}{z^2} \end{bmatrix} \\
    %
    %
    %
    \mathbf{H}_{\theta_k} &=  \mathbf{H}_{proj} {}^C_I\mathbf{R} \lfloor {}^{I_k}_G\mathbf{R}\left( {}^G \mathbf{p}_M + {}^M_G \mathbf{R}^{\top} {}^M \mathbf{L}_f- {}^G\mathbf{p}_{I_k} \right) \rfloor \\
    %
    %
    %
    \mathbf{H}_{p_k} &= - \mathbf{H}_{proj} {}^C_I\mathbf{R} {}^{I_k}_G\mathbf{R} \\
    %
    %
    %
       \mathbf{H}_{\psi} &= - \mathbf{H}_{proj} {}^C_I\mathbf{R} {}^{I_k}_G\mathbf{R} {}^M_G \mathbf{R}^{\top} \lfloor {}^M \mathbf{L}_f \rfloor \mathbf{e}_z \\
       %
       %
       %
        \mathbf{H}_{p_M} &= \mathbf{H}_{proj} {}^C_I\mathbf{R} {}^{I_k}_G\mathbf{R}
\end{align}
where $\mathbf{e}_z = \begin{bmatrix} 0 & 0 & 1 \end{bmatrix}^{\top}$.

In order to obtain an initial estimate of this map transformation we collect bearing measurements to known landmarks over a window. By fixing the robot state estimates, we can perform linear triangulation for the landmarks that have been observed. After obtaining estimates for the landmarks in both the global and map frames, we can use standard techniques to find the 6 DOF relative transformation. We then extract the yaw and relative position from this solution. This then serves as the initial values of the map transformation for use in delayed initialization. 

